Prompt-responsive Object Retrieval with Memory-augmented Student-Teacher Learning

Building models responsive to input prompts represents a transformative shift in machine learning. This paradigm holds significant potential for robotics problems, such as targeted manipulation amidst clutter. In this work, we present a novel approach to combine promptable foundation models with reinforcement learning (RL), enabling robots to perform dexterous manipulation tasks in a prompt-responsive manner. Existing methods struggle to link high-level commands with fine-grained dexterous control. We address this gap with a memory-augmented student-teacher learning framework. We use the Segment-Anything 2 (SAM 2) model as a perception backbone to infer an object of interest from user prompts. While detections are imperfect, their temporal sequence provides rich information for implicit state estimation by memory-augmented models. Our approach successfully learns prompt-responsive policies, demonstrated in picking objects from cluttered scenes. Videos and code are available at https://memory-student-teacher.github.io

==> figures/hardware_setup.tex <==
\begin{figure}[t]
		\includegraphics[width=\linewidth]{example-image}
	\caption{\textbf{Hardward setup.} The robot used in this work combines a Universal Robot UR5 arm and Schunk SIH hand.}
	\label{fig:hardware_setup}
\end{figure}

==> figures/rollouts/rollouts.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth, height=6cm]{example-image}  
	\caption{Teaser caption.}
	\label{fig:teaser}
  \end{figure}



==> figures/student_architecure/student_architecture.tex <==
\begin{figure*}[t]
    \centering
    
    \begin{subfigure}{0.495\linewidth}
      \includegraphics[width=\linewidth, height=6cm]{example-image}  
      \caption{Encoder Architecture.}
      
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.245\linewidth}
      \includegraphics[width=\linewidth, height=6cm]{example-image}  
      \caption{Transformer.}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.245\linewidth}
      \includegraphics[width=\linewidth, height=6cm]{example-image}  
      \caption{Contextformer.}
    \end{subfigure}
	\caption{\textbf{Student architecture.} }
	\label{fig:student_architecture}
  \end{figure*}
  
  
